ViTGAN: Training GANs with Vision Transformers

Recently, Vision Transformers (ViTs) have shown competitive performance on image recognition while requiring less vision-specific inductive biases. In this paper, we investigate if such performance can be extended to image generation. To this end, we integrate the ViT architecture into generative adversarial networks (GANs). For ViT discriminators, we observe that existing regularization methods for GANs interact poorly with self-attention, causing serious instability during training. To resolve this issue, we introduce several novel regularization techniques for training GANs with ViTs. For ViT generators, we examine architectural choices for latent and pixel mapping layers to facilitate convergence. Empirically, our approach, named ViTGAN, achieves comparable performance to the leading CNN-based GAN models on three datasets: CIFAR-10, CelebA, and LSUN bedroom.

==> figures/table1_lu_old.tex <==
\begin{table}[t]
\vspace{-1em}
\setlength{\tabcolsep}{0.5em}
\renewcommand{\arraystretch}{1.1}
	\centering
	\small
\begin{tabular}{@{}lcccccccc@{}}
\hline
\toprule
\multirow{2}{*}{\textbf{Architecture}} & \multirow{2}{*}{\textbf{Conv}}  & \multirow{2}{*}{\textbf{Pool}} & \multicolumn{2}{c}{\textbf{CIFAR}} & \multicolumn{2}{c}{\textbf{CelebA}}& \multicolumn{2}{c}{\textbf{LSUN Bedroom}} \\ \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
                       & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \textbf{FID $\downarrow$} & \textbf{IS $\uparrow$} & \textbf{FID $\downarrow$} & \textbf{IS $\uparrow$} & \textbf{FID $\downarrow$} & \textbf{IS $\uparrow$}\\ 
\midrule
BigGAN+ DiffAug\footnotesize{~\citep{zhao2020diffaugment}}   & \ck & \ck &  8.59\textsuperscript{$\ast$}  & 9.25\textsuperscript{$\ast$}   &  -   & -   &  - &  - \\
StyleGAN2\footnotesize{~\citep{Karras2019stylegan2}} & \ck & \ck & 11.1\textsuperscript{$\ast$}   & 9.18\textsuperscript{$\ast$} & \textbf{3.39}  & \textbf{3.43}  & 3.25     & \textbf{2.45} \\
\midrule
TransGAN-XL\footnotesize{~\citep{jiang2021transgan}}& \xk & \ck & 11.9\textsuperscript{$\ast$} & 8.63\textsuperscript{$\ast$}  & -   & -  & -  &  - \\
Vanilla-ViT  & \xk & \xk & 12.7         & 8.40  &  20.2    &  2.57  &  218.1     &  2.20  \\
%Transformer G(B) + ViT D    & N        & -      & -      &      &   &    &   \\ 
\midrule
ViTGAN (Ours)  & \xk & \xk & \textbf{6.66} & \textbf{9.30} & 3.74  & 3.21  & \textbf{2.65}  &  2.36    \\

%ViTGAN (Ours)  & N & Y & N/A & N/A & \textbf{3.96}  & 3.06  & \textbf{2.84}  &  2.29    \\
\bottomrule
\hline
\end{tabular}
\vspace{2mm}
\caption{\textbf{Comparison to representative GAN architectures on unconditional image generation benchmarks.}
\textsuperscript{$\ast$}Results from the original papers. All other results are our replications. ‘Conv’, and ‘Pool’ stand for convolution, and pooling (\ie, downsampling or upsampling), respectively. $\downarrow$ means lower is better. $\uparrow$ means higher is better.
}
	%\vspace{-1em}
\label{table:main_results}
\end{table}

==> figures/table6_vit_mlp.tex <==
\begin{wraptable}{r}{0.6\textwidth}
\vspace{-1em}
\caption{\label{tab:vit_mlp}\textbf{MLP-mixer, ViT, ViT+local attn, ViT+CvT}. 
%Even paired with CNN generators or discriminators, our mixed ViTGAN can still achieve reasonable performance 
%on CIFAR-10.
%All the models are trained with bCR + DiffAug.
}
\footnotesize
%\setlength{\tabcolsep}{0.5em}
\vspace{-3mm}
%\renewcommand{\arraystretch}{1.1}
	\centering
	\begin{tabular}{@{}lccc@{}cc@{}}
	\hline
	\toprule
	\textbf{Method} & \textbf{attention}  & \textbf{local}  & \textbf{global} & \normalsize{} \textbf{CIFAR FID $\downarrow$} & \normalsize{} \textbf{LSUN FID $\downarrow$} \tabularnewline
	\midrule
	\normalsize{} StyleGAN2 & \normalsize{} \xk & \ck & \xk & \normalsize{} 5.60 & \normalsize{} 2.59 \tabularnewline
    \midrule
    \normalsize{} ViT & \normalsize{} \ck & \xk & \ck & \normalsize{}  6.66 & \normalsize{} 1.94 \tabularnewline
	\normalsize{} MLP-Mixer & \normalsize{} \xk & \xk  & \ck & \normalsize{} {8.93} & \normalsize{} {3.23} \tabularnewline
	\normalsize{} ViT-local & \normalsize{} \ck & \ck & \xk & \normalsize{} \textbf{{4.76}} & \normalsize{} {1.79} \tabularnewline
	\midrule
	\normalsize{} ViTGAN & \normalsize{} \ck & \ck & \ck & \normalsize{} {4.92} & \normalsize{} {\textbf{1.57}} \tabularnewline
	\bottomrule
	\hline
\end{tabular}
	%\vspace{2mm}
	%\vspace{-1em}
\end{wraptable}
